Recurrent Neural Network Regularization

We present a simple regularization technique for Recurrent Neural Networks (RNNs) with Long Short-Term Memory (LSTM) units. Dropout, the most successful technique for regularizing neural networks, does not work well with RNNs and LSTMs. In this paper, we show how to correctly apply dropout to LSTMs, and show that it substantially reduces overfitting on a variety of tasks. These tasks include language modeling, speech recognition, image caption generation, and machine translation.

==> Makefile <==
PARTS=rnn.tex

all: clean rnn.pdf 

rnn.pdf: $(PARTS) bibliography.bib 
	pdflatex -shell-escape rnn.tex
	pdflatex -shell-escape rnn.tex
	pdflatex -shell-escape rnn.tex
	bibtex rnn
	bibtex rnn
	bibtex rnn
	pdflatex -shell-escape rnn.tex
	pdflatex -shell-escape rnn.tex

clean:
	rm -f *.log *.blg *.aux *.bbl *.4tc *.xref *.tmp *.dvi *.hd *.idx *.out *.toc *.drv *.ins *.py *.pdf
	rm -rf ~*
	rm -rf *.tmp
	rm -rf *.4om
	rm -rf *~

tar:
	find . -type f | egrep -v '\.git|\.log|\.swp' | xargs tar zcvf ../rnn_reg.tar.gz

